Revisiting Fuzzy Signatures: Towards a More Risk-Free Cryptographic Authentication System based on Biometrics

Biometric authentication is one of the promising alternatives to standard password-based authentication offering better usability and security. In this work, we revisit the biometric authentication based on "fuzzy signatures" introduced by Takahashi et al. (ACNS'15, IJIS'19). These are special types of digital signatures where the secret signing key can be a "fuzzy" data such as user's biometrics. Compared to other cryptographically secure biometric authentications as those relying on fuzzy extractors, the fuzzy signature-based scheme provides a more attractive security guarantee. However, despite their potential values, fuzzy signatures have not attracted much attention owing to their theory-oriented presentations in all prior works. For instance, the discussion on the practical feasibility of the assumptions (such as the entropy of user biometrics), which the security of fuzzy signatures hinges on, is completely missing. In this work, we revisit fuzzy signatures and show that we can indeed efficiently and securely implement them in practice. At a high level, our contribution is threefold: (i) we provide a much simpler, more efficient, and direct construction of fuzzy signature compared to prior works; (ii) we establish novel statistical techniques to experimentally evaluate the conditions on biometrics that are required to securely instantiate fuzzy signatures; and (iii) we provide experimental results using a real-world finger-vein dataset to show that finger-veins from a single hand are sufficient to construct efficient and secure fuzzy signatures. Our performance analysis shows that in a practical scenario with 112-bits of security, the size of the signature is 1256 bytes, and the running time for signing/verification is only a few milliseconds.

==> Input_Sections/Hardness_DLwSketch.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US


\section{Security of the \DL Assumption with Sketch $(\DLsketch)$} \label{app_sec:analysis_dlsketch}
For reference, we provide again the two facts which we use to argue the hardness of the $\DLsketch$ assumption:
\begin{enumerate}
\item If $\CFMR \lessapprox 2^{-(2 \secpar + \omega(\log \secpar))}$, then the standard $\DL$ assumption implies the $\DLsketch$ assumption;
\item If $\CFMR \approx 2^{-\secpar}$ (or even $2^{-\omega(\log \secpar)}$), then the $\DLsketch$ assumption holds in the generic group model \cite{EC:Shoup97}. 
\end{enumerate}
In this section, we give an explanation for each item.
To explain, we use the following notions:
Recall that for a joint distribution $(\mathcal{X}, \mathcal{C})$, the (average) \emph{conditional collision entropy} of $\mathcal{X}$ given $\mathcal{C}$ is defined by $\avgcollentropy(\mathcal{X}|\mathcal{C}) := - \log_2 \COL(\mathcal{X}|\mathcal{C})$, where
{\small
\begin{equation}
\COL(\mathcal{X}|\mathcal{C})
:= \Pr[(x,c), (x', c') \samp (\mathcal{X}, \mathcal{C}) : x = x' | c = c']. \label{eqn:CR}
\end{equation}
}
Here, $\COL(\mathcal{X}|\mathcal{C})$ is called the \emph{conditional collision probability of $\mathcal{X}$ given $\mathcal{C}$}.
When the context is clear, 
we often abuse notation and write $\avgcollentropy(x|c)$ instead of $\avgcollentropy(\mathcal{X}|\mathcal{C})$, and we do a similar treatment for $\COL$. 


\noindent{\underline{\textit{(1) $\DL$ implies $\DLsketch$ when $\CFMR$ is sufficiently small.}}}
Identifying the joint distribution $(\mathcal{X}, \mathcal{C})$ in \cref{eqn:CR} with $\{\vx \samp \FuzDataDist : (\vx, \vc = \vx - g_{\Lattice}(\vx)) \}$, we clearly have $\COL(\vx|\vc) \le \CFMR$.
Moreover, observe $\COL(\vx|\vc) = \COL(\mB^{-1} \vy|\vc)$, since recovering $\vx$ given $\vc$ implies recovering $\mB^{-1} \vy$ given $\vc$ and vice versa due to $\vc = \vx - \vy$. 
Now, suppose we had an upper bound of $\COL(\mB^{-1}\vy|\vc) \le p^{-1} \cdot 2^{-\omega(\log \secpar)}$, or equivalently $\avgcollentropy(\mB^{-1}\vy|\vc) \ge \log_2 p + \omega(\log \secpar)$, when we sample $\vx \samp \FuzDataDist$ and calculate $(\vc, a) \lruns \Sketch(\LinSpp, \vx)$, where $\vc = \vx - \vy = \vx - g_{\Lattice}(\vx)$.
Then, the leftover hash lemma of \cite{SICOMP:DORS08}, formally recalled in \cref{app_sec:lhl}, guarantees that the proxy key $a = \linhash(\mB^{-1} \vy) \in \ZZ_p$ is statistically close to a uniformly random element even given $\vc$, and thus the standard $\DL$ assumption implies the $\DLsketch$ assumption.

Putting things together, if $\CFMR \lessapprox 2^{-(2 \secpar + \omega(\log \secpar))}$, then  standard $\DL$ implies the $\DLsketch$ assumption since $p \approx 2\secpar$.
However, since typically $\secpar \ge 80$, this condition on $\CFMR$ may be somewhat too expensive to assume for fuzzy biometrics. 
Nevertheless, we believe the above provides us an intuition that the $\DLsketch$ assumption is not an esoteric assumption and justifies that $\CFMR$ is the right quantity to care about.


\noindent{\underline{\textit{(2) $\DLsketch$ is hard in the generic group model.}}
The generic group model \cite{EC:Shoup97} is an idealized model of computation for a cyclic group, where algorithms do not use the representation (or, the encoding) of the group elements, other than testing the equality of group elements.
When a new computational problem related to a cyclic group is introduced, this model is typically used to reason about its hardness.
Specifically, if some computational problem is proved to be hard for PPT adversaries in the generic group model, then it formally guarantees that one cannot solve the problem efficiently as long as one is performing only group operations.
To solve it efficiently, one must rely on a weakness of a particular group.
Thus, the hardness of a computational problem in the generic group model serves as a strong evidence that if we use a cyclic group where no such weakness is known (e.g. a group over an elliptic curve).


Based on existing works, we can observe that if $\CFMR \approx 2^{-\secpar}$ (or even $2^{-\omega(\log \secpar)} = \secpar^{-\omega(1)}$), then there is no PPT algorithm that can break the $\DLsketch$ assumption in the generic group model.
Specifically, it is a well-known fact (and formally shown in \cite[Lemma 6]{TCC:DodYu13}) that a universal hash family is a good \lq\lq strong randomness condenser'' and preserves essentially all the (conditional) collision entropy of the input $\mB^{-1}\vy$ of $\linhash$ to its output $a = \linhash(\mB^{-1}\vy)$.
That is, we have $\COL(a|\linhash,\vc) \approx \COL(\mB^{-1}\vy|\vc) \le \CFMR$.
Moreover, \cite{C:BitCan10} considers a stronger variant of the decisional Diffie-Hellman problem where the exponents are not uniformly distributed but of superlogarithmic min-entropy $\omega(\log \secpar)$, and showed that this problem is hard for any PPT adversary in the generic group model.
This directly implies the hardness of the $\DL$ problem in which the exponent of a problem instance is chosen from a distribution with min-entropy $\omega(\log \secpar)$ in the generic group model.
Finally, min-entropy and collision entropy are linearly related.
Hence, taking average over the choice of $\vc = \vx - \vy$, we can conclude that the $\DLsketch$ problem is hard to solve for any PPT adversary in the generic group model if $\CFMR = 2^{-\omega(\log \secpar)}$.




==> Input_Sections/LHL.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\section{Leftover Hash Lemma} \label{app_sec:lhl}

Here we recall the leftover hash lemma of \cite{SICOMP:DORS08}.
To see the connection with the explanation in \cref{sec:analysis_dlsketch}, we state it using conditional collision probability.

Recall that for a joint distribution $(\mathcal{X}, \mathcal{Y})$, the (average) conditional collision probability of $\mathcal{X}$ given $\mathcal{Y}$ is defined by $\COL(\mathcal{X}|\mathcal{Y}) = \Pr_{(x,y), (x', y') \samp (\mathcal{X}, \mathcal{Y})}[x = x' | y = y']$.

Recall also that the statistical distance between two distributions $\mathcal{X}$ and $\mathcal{Y}$
is defined by
$\SD(\mathcal{X}, \mathcal{Y}) := \frac{1}{2} \sum_{z}\abs{\Pr[\mathcal{X} = z] - \Pr[\mathcal{Y} = z]}$.
It is known that $\SD(\mathcal{X}, \mathcal{Y})$ upper-bounds the best (computationally unbounded) adversary's advantage in distinguishing the distribution using a single sample.

\begin{lemma}[Slightly adapted from \cite{SICOMP:DORS08}]
Let $\linHashFamily = \{\linhash: D \to R\}$ be a family of universal hash functions.
Let $\mathcal{X}$ and $\mathcal{Y}$ be distributions such that $(\mathcal{X}, \mathcal{Y})$ forms a joint distribution, and the support of $\mathcal{X}$ is contained in $D$.
Then, the statistical distance of the following two distributions is at most $\frac{1}{2} \sqrt{|R| \cdot \COL(\mathcal{X}|\mathcal{Y})}$:
\begin{align*}
&\bigl\{ \linhash \samp \linHashFamily;~ (x, y) \samp (\mathcal{X}, \mathcal{Y}): (\linhash, \linhash(x), y) \bigr\},\\
&\bigl\{ \linhash \samp \linHashFamily;~ (x, y) \samp (\mathcal{X}, \mathcal{Y});~ r \samp R: (\linhash, r, y) \bigr\}.
\end{align*}
In particular, if $\COL(\mathcal{X}|\mathcal{Y}) \le |R|^{-1} \cdot 2^{-\omega(\log \secpar)}$, then the statistical distance is $\negl(\secpar)$.
\end{lemma}

Strictly speaking, \cite{SICOMP:DORS08} showed the above lemma using the (average) conditional min-entropy (rather than conditional collision entropy/probabiltiy).
However, the above lemma can be easily inferred from the proof of \cite[Lemma~2.4]{SICOMP:DORS08} and the fact that the most basic form of the leftover hash lemma \cite{HILL99} (without taking into account the existence of $\mathcal{Y}$) works with collision entropy.



